SAGE: A Self-Evolving Agentic Graph-Memory Engine for Structure-Aware Associative Memory

Long-term memory is becoming a central bottleneck for language agents. Exsting RAG and GraphRAG systems largely treat memory graphs as static retrieval middleware, which limits their ability to recover complete evidence chains from partial cues, exploit reusable graph-structrual roles, and improve the memory itself through downstream feedback. We introduce SAGE, a Self-evolving Agentic Graph-memory Engine that models graph memory as a dynamic long-term memory substrate. SAGE couples two roles: a memory writer that incrementally constucts structured graph memory from interaction histories, and a Graph Foundation Model-based memory reader to perform retrieval and provide feedback to the memory writer. We provide rigorooous theoretical annalyses supporting the framework. Across multi-hop QA, open-domain retireval, domain-specific review QA, and long-term agent-memory benchmarks, SAGE improves evidence recovery, answer grounding, and retrieval efficiency: after two self-evolution rounds, it achieves the best average rank on multi-hop QA; in zero-shot open-domain transfer, it reaches 82.5/91.6 Recall@2/5 on NQ. Further results on LongMemEval and HaluMem show that traning and reader-writer feedback improve multiple long-term memory and hallucination-diagnostic metrics, suggesting that self-evolving, structure-aware graph memory is a promising foundation for robust long-horizon language agents.

==> 04-2-1_opendomain_results.tex <==
% \subsection{标准 open-domain RAG}

% 这层是为了和更广义的 RAG 方法对齐，避免文章只在多跳窄赛道中比较。加入：
% \begin{itemize}
%     \item Natural Questions (NQ)；
%     \item TriviaQA；
%     \item PopQA；
%     \item ASQA；
%     \item MultiHop-QA
% \end{itemize}


%1.0-shot

%HotpotQA + 2WikiMultiHopQA + MuSiQue 上训练我们的 constructor / retriever 自进化闭环；然后不在 NQ、TriviaQA、PopQA、ASQA、CLAPnQ 上做任何梯度更新，直接 zero-shot 测。这样你测到的是“一个从多跳结构化记忆任务中学出来的 memory system，能不能泛化到更广义 open-domain / long-form RAG”。这正好服务你“不是又一个 GraphRAG，而是 self-evolving memory system”的主线。这个主表里，NQ / TriviaQA / PopQA 是短答案 OOD transfer，ASQA / CLAPnQ 是长答案 grounded OOD transfer。
\input{knowledge-intensive}


%非必要，做了可以丢附录
% 2.Target-domain continual adaptation / self-evolution
% 在 zero-shot 之后，给每个目标数据集一个很小的 adaptation budget，例如只用 train split 的一个小子集，或者 1–2 轮 alternating improvement，然后再测 test。报告：

% zero-shot
% +1 round adaptation
% +2 rounds adaptation

% 这张表最能体现你的方法和普通 RAG baseline 的区别，因为你不是只会“迁移”，而是会继续学会在新领域中该记什么、如何重组记忆索引。这和 HippoRAG 2 把 NQ / PopQA 当 factual memory、再和多跳任务一起看 continual learning 的做法是同一方向，只是你更强调 writer–reader co-evolution。


% 3.In-domain upper bound
% 分别在 NQ / TriviaQA / PopQA / ASQA / CLAPnQ 上做 in-domain training 或 continued evolution，给一个 upper bound。这样 reviewer 就没法说你“只会跨域 zero-shot，但本域上限不清楚”。




==> 04-2-2_amazon_results.tex <==
% \subsection{GraphRAG 与 domain-specific}

% 这层专门服务于图索引与图推理卖点。建议包含：
% \begin{itemize}
%     \item GRBench-e-commerce / Amazon domain slice；
%     \item AmazonQA（或其图化版本 / 图引导检索版本）。
% \end{itemize}
% GRBench 直接评估文本图推理与 graph-augmented reasoning，GraphRAG-Bench 强调 GraphRAG 的全流程评测，AmazonQA 则提供真实噪声评论场景下的 review-based QA~\citep{graphcot2024,graphragbench2025,amazonqa2019}。


% 1.AmazonQA：
% 是 2019 年提出的 review-based QA benchmark，规模很大：923k questions、3.6M answers、14M reviews、156k products，并且额外标了answerable / unanswerable。这是它和很多普通 QA 数据最不一样的地方：问题、评论、答案都来自真实电商用户交互。原始 AmazonQA 论文的经典表是 BLEU-4 + ROUGE，重点在“给 reviews + 问题，生成一个 answer”。

% 使用为与旧文献对齐的 legacy 指标
% BLEU-4
% ROUGE / ROUGE-L

% zero-shot：仍然先用只在 HotpotQA、2Wiki、MuSiQue 上训练好的系统直接测
% + 小预算 adaptation：因为 AmazonQA 的 domain shift 很大，answer style 也更自由，仅看 zero-shot 容易低估你的系统。



\input{Amazonqa}






% 2.GRBench 的 e-commerce / Amazon domain slice
% Graph-CoT 论文引入的 GRBench 总共有 1,740 个问题、10 个 domain graphs、5 个大域。后续 GraphDancer 则给出了一个更细的 cross-domain 设定：只在 Academic 域训练，在 E-commerce、Literature、Healthcare、Legal 上测试；它的 Table 1 还显示 E-commerce split 有 200 个问题：80 Easy、40 Medium、40 Hard、40 OOD。Graph-CoT / Graph-O1 / GraphDancer 多是 ROUGE-L + GPT4Score；
% Inference Scaled GraphRAG 报的是 F1；
% GraphRunner / Grounding-KG 在公开摘要里更多报的是相对提升和成本下降。

% 主 setting：
% 只在 HotpotQA + 2Wiki + MuSiQue 上训练 graph constructor / GFM retriever / self-evolving loop
% 不在 GRBench-Amazon 上做参数更新，先 zero-shot 测


% 第二张表我建议模仿 GraphDancer 再做一个：
% cross-domain adaptation / one-round self-evolution
% 例如 train on Academic-style graph memories，adapt 少量 E-commerce data，再测 E-commerce
% GraphDancer 已经证明这种 train-one-domain, test-unseen-domains 的设定很有说服力。



\input{GRBench}



==> 04-2_main_multihop_results.tex <==

% \subsection{核心多跳 RAG}
% 包含：
% \begin{itemize}
%     \item HotpotQA；
%     \item 2WikiMultiHopQA；
%     \item MuSiQue；
%     \item Bamboogle；
%     \item MultiHop-RAG。
% \end{itemize}

% 其中 HotpotQA、2Wiki 和 MuSiQue 是当前多跳 / iterative RAG 的主流公共基准，GFM-RAG、DeepRAG、FrugalRAG、Q-RAG 等方法都直接或间接围绕这类任务展开~\citep{gfmrag2025,deeprag2025,frugalrag2025,qrag2025,multihoprag2024}。Bamboogle 可以作为更难、更偏组合性的信息寻求测试；MultiHop-RAG 则能提供显式 supporting evidence，对后续定义 \gsr\ 与 path-level recall 很有帮助~\citep{multihoprag2024}。








\input{multi_retrieve}


==> 04-3_self_evolving_memory.tex <==

% \section{本章的地位}

% 如果说上一章证明了 \method\ “能用”，那么这一章要证明它“\textbf{为什么值得被称为自进化记忆系统}”。这也是整篇论文最重要的概念性实验章节。强烈建议至少给一张 evolution curve 主图和两张控制实验表。

% \section{实验 5：constructor--retriever 闭环共演化曲线}

% \subsection{实验设计}

% 设 $\constructor_t$ 与 $\retriever_t$ 表示第 $t$ 轮的写入器与读取器。运行：
% \[
% (\constructor_0,\retriever_0)\rightarrow
% (\constructor_1,\retriever_1)\rightarrow
% (\constructor_2,\retriever_2)\rightarrow \cdots
% \]
% 每轮都重新构图或做增量图更新，然后在固定验证集上评测。

% \subsection{必须报告的指标}

% \begin{itemize}
%     \item EM / F1；
%     \item \gsr\ 与 \gpc{}@k；
%     \item Recall@k；
%     \item 平均检索轮数 / latency；
%     \item 图规模（节点、边、激活子图大小）；
%     \item Utility Density：单位图预算对应的性能收益。
% \end{itemize}

% \subsection{图表形式}

% 最少放两张图：
% \begin{itemize}
%     \item \textbf{性能随轮数变化曲线}；
%     \item \textbf{图质量随轮数变化曲线}（如 \gsr{}、unsupported edge rate、子图稀疏度）。
% \end{itemize}

% \subsection{你需要的结论模式}

% \begin{itemize}
%     \item 完整闭环在前 2--3 轮持续提升，而不是第一轮后立刻饱和；
%     \item 图质量提升与最终 QA 提升同步发生；
%     \item 图规模未必单调增大，甚至可能更稀疏，但 utility density 上升。
% \end{itemize}

% \section{实验 6：单边更新 vs 联合更新 vs 一次性训练}

% 这是 reviewer 一定会问的控制实验。建议做如下对照：

% \begin{itemize}
%     \item 只更新 \constructor，固定 \retriever；
%     \item 只更新 \retriever，固定 \constructor；
%     \item 联合单轮训练（无多轮闭环）；
%     \item 完整多轮闭环；
%     \item oracle graph 或 oracle retriever 上界。
% \end{itemize}

% \subsection{想证明什么}

% \begin{enumerate}
%     \item 只训 retriever 能提升读取，但天花板较低；
%     \item 只训 constructor 能改善图，但无法完全兑现为检索收益；
%     \item 一次性 joint train 可以带来初步收益，但不如多轮闭环稳定；
%     \item 完整 co-evolution 才能持续提升写入器与读取器的耦合质量。
% \end{enumerate}

% \section{实验 7：stability--plasticity}

% “自进化”最怕被 reviewer 质疑为“逐轮过拟合或灾难性遗忘”，所以必须补这组实验。

% \subsection{实验设置}

% \begin{itemize}
%     \item 阶段 1：在 HotpotQA / MuSiQue 上训练若干轮；
%     \item 阶段 2：引入新域，如 AmazonQA、GRBench-Amazon 或 LongMemEval 的知识更新子集；
%     \item 测试：同时评估旧域表现与新域适应表现。
% \end{itemize}

% \subsection{指标}

% \begin{itemize}
%     \item 新域提升（plasticity）；
%     \item 旧域保持率（stability / retention）；
%     \item latest fact accuracy；
%     \item stale-memory error rate；
%     \item 你可以定义一个 Stability--Plasticity Index 作为综合指标。
% \end{itemize}

% \subsection{结果应该如何解释}

% 你希望看到的是：\method\ 不仅在新域上继续变强，而且对旧域的损伤更小。这能支撑“自进化”不是简单重写全部记忆，而是更像有组织地吸收新经验。





% \section{本章写作提醒}

% \begin{itemize}
%     \item 千万不要把“自进化”只写成一行口号，必须用\textbf{曲线}呈现。
%     \item 要主动承认：收益通常不会无限增长，过多轮数可能出现平台期；这反而显得真实。
%     \item 最好给一个 qualitative case，展示第 0 轮和第 3 轮的图差异：哪些冗余边消失，哪些桥接边保留，哪些错误边被修正。
% \end{itemize}


==> 04-4_agent_memory_results.tex <==



% LongMemEval 官方提供三个文件：LongMemEval_S、LongMemEval_M、LongMemEval_oracle，每个文件都有 500 个 evaluation instances；S 大约是 115k tokens / 约 40 个 session，M 大约 500 个 session，oracle 只保留证据 session。任务覆盖 6 类问题：single-session-user、single-session-assistant、single-session-preference、temporal reasoning、knowledge update、multi-session。

% \section{实验 10：LongMemEval 全套评测}

% LongMemEval 专门覆盖五类能力：信息提取、多 session 推理、时间推理、知识更新与 abstention~\citep{longmemeval2024}。这正适合用来展示你的系统不是单纯 document retriever，而是会随着历史积累形成结构化可检索记忆。



\input{LongMemEval}




% \section{实验 11：HaluMem 上的 operation-level 幻觉分析}

% HaluMem 是一个operation-level memory hallucination benchmark，不是单纯 QA benchmark。它专门把 memory system 拆成三段：memory extraction、memory updating、question answering，并分别统计 correct / hallucination / omission 等指标。它有两个主集：HaluMem-Medium 和 HaluMem-Long。官方 repo 给出的规模是：Halu-Medium 有 20 个用户、30,073 段对话、平均 70 sessions/user、约 160k tokens、14,948 memory points 和 3,467 QA；Halu-Long 则是 53,516 段对话、平均 120 sessions/user、约 1M tokens，memory points 和 QA 数相同。

% \subsection{主实验}

% \begin{itemize}
%     \item 使用 benchmark 原生的 extraction / updating / QA 三类任务；
%     \item 额外报告图级指标：
%     \begin{itemize}
%         \item Unsupported Node Rate；
%         \item Unsupported Edge Rate；
%         \item Stale Edge Rate；
%         \item Contradiction Propagation Rate。
%     \end{itemize}
% \end{itemize}

% \subsection{要比较的 baselines}

% \begin{itemize}
%     \item raw long-context；
%     \item extractive memory；
%     \item summary memory；
%     \item vector memory；
%     \item graph memory without RL；
%     \item \method{}。
% \end{itemize}

% \subsection{你想证明什么}

% \begin{enumerate}
%     \item 幻觉并不只发生在最终回答阶段，而会在记忆写入阶段被放大；
%     \item 你的双 reward 特别是 $\rc$，有助于抑制“无支撑但看似有用”的虚假边；
%     \item 较低的 graph hallucination rate 会转化为较低的 downstream QA hallucination。
% \end{enumerate}




==> Training_Inference_Complexity.tex <==
\section{Training and Inference Complexity}
\label{app:complexity}

For ease of exposition, suppose that the graph
$\mathcal{G}=(\mathcal{V},\mathcal{E})$ has $n=|\mathcal{V}|$ entity nodes and
$m=|\mathcal{E}|$ entity-relation edges. If self-loops are added in GCN propagation, we denote
$\tilde m=m+n$. Let the hidden dimension be $d$, the number of propagation layers be $L$, the batch size be $B$, and the number of pseudo-queries be $M$.
Therefore, one real query together with $M$ pseudo-queries requires $M+1$ graph reads. Let $\mathbf{M}\in\{0,1\}^{n\times N_D}$
denote the sparse entity--document association matrix, where $N_D$ is the number of documents, and $\operatorname{nnz}(\mathbf{M})$ is the number of nonzero entity--document links.
Let $K_e$ denote the number of top entities used for document projection, and let $\bar f$ denote the average number of documents linked to the top entities.

\subsection{Offline Structural Feature and Indexing Cost}
\label{app:complexity_offline}

Let the dimension of node structural features be $p_n$, the dimension of edge structural features
be $p_e$, and the dimension of graph-level summaries be $p_g$. In the current implementation, $p_n$, $p_e$, and $p_g$ are all small constants.

Given that the adjacency list has been constructed, degrees and average neighbor degrees can be computed in $O(n+m)$ time. Clustering coefficients and the number of common neighbors require computing intersections of neighbor
sets, whose complexity can be written as
\begin{equation}
    O\left(
    n+m+
    \sum_{(u,v)\in\mathcal{E}}
    \min\{\deg(u),\deg(v)\}
    \right).
    \label{eq:structure_feature_cost}
\end{equation}
In sparse graphs or graphs with bounded average degree, Eq.~\eqref{eq:structure_feature_cost} is approximately $O(n+m)$; in extremely dense graphs,
the worst case can reach $O(n^3)$. These structural features and the entity--document matrix can both be precomputed and cached offline, with space cost
\begin{equation}
    O\left(np_n+mp_e+p_g+\operatorname{nnz}(\mathbf{M})\right).
\end{equation}
Since this part does not depend on a specific query, when evaluating multiple queries on the same candidate graph in the self-evolving memory loop,
the same set of structural features and entity--document indices can be reused.

\subsection{Forward Propagation Complexity of the Structurally Gated GFM}
\label{app:complexity_gfm_forward}

We first consider a single forward propagation for one query on one graph. A standard GCN layer contains two parts: node linear transformation and sparse adjacency aggregation.
The cost of node linear transformation is $O(nd^2)$, and the cost of edge-level message aggregation is $O(\tilde m d)$. Therefore, the complexity of a standard GCN layer is
\begin{equation}
    C_{\mathrm{plain}}
    =
    O\left(nd^2+\tilde m d\right).
    \label{eq:plain_gcn_complexity}
\end{equation}

Beyond ordinary message propagation, a structurally gated layer generates a vector gate for each edge. Its message form is
\begin{equation}
    \mm_{u\rightarrow v}
    =
    \gg_{uv}\odot W\hh_u,
\end{equation}
where $\hh_u$ is the source node representation, $W\in\mathbb{R}^{d\times d}$ is the node linear transformation matrix,
$\gg_{uv}\in\mathbb{R}^{d}$ is the structural gate vector of edge $(u,v)$, and $\odot$ denotes element-wise multiplication.
Let $d_g$ denote the encoding dimension of structural features, and let $h_g$ denote the hidden dimension of the gating MLP. If the gate uses four types of inputs, namely source-node structure, target-node structure,
edge-pair structure, and graph-level summary, then the gate generation cost can be written as
\begin{equation}
\begin{aligned}
    C_{\mathrm{gate}}
    =
    O\Big(
        &np_n d_g
        + mp_e d_g
        + p_g d_g  \\
        &+ m(4d_g h_g + h_g d)
    \Big).
\end{aligned}
\label{eq:gate_complexity}
\end{equation}
Here, $np_n d_g$ comes from node structural feature encoding, $mp_e d_g$ comes from edge structural feature encoding, $p_g d_g$ comes from graph-level summary encoding,
and $m(4d_g h_g+h_g d)$ comes from the per-edge gating MLP. If edge-pair features or graph-level summaries are disabled, the corresponding terms in Eq.~\eqref{eq:gate_complexity}
can be removed. If $d_g$ and $h_g$ are regarded as being of the same order as $d$, then gate generation is
$O(md^2)$ in the worst case; if the gating MLP is regarded as a small constant-width module, or if low-rank/dimension-wise gating is adopted, it can be approximated as $O(md)$.
Therefore, the complexity of a structurally gated layer is
\begin{equation}
    C_{\mathrm{gated}}
    =
    O\left(nd^2+\tilde m d+C_{\mathrm{gate}}\right).
    \label{eq:gated_layer_complexity}
\end{equation}

The current implementation supports dual structural prompts: one is a holistic gated branch, and the other is a specific prompt branch. If only a standard GCN is used,
the per-layer cost is $C_{\mathrm{plain}}$; if only a structurally gated GCN is used, the per-layer cost is
$C_{\mathrm{gated}}$; if one gated branch and one standard branch are used simultaneously, the per-layer cost is approximately
$C_{\mathrm{gated}}+C_{\mathrm{plain}}$. Let $\rho_{\mathrm{plain}}\in\{0,1\}$ denote whether the standard prompt branch is enabled,
and let $\rho_{\mathrm{gated}}\in\{0,1\}$ denote whether the structurally gated branch is enabled. Then the GFM encoding cost for one batch can be uniformly written as
\begin{equation}
    C_{\mathrm{enc}}(B)
    =
    O\left(
    B L
    \left(
    \rho_{\mathrm{plain}} C_{\mathrm{plain}}
    +
    \rho_{\mathrm{gated}} C_{\mathrm{gated}}
    \right)
    \right).
    \label{eq:encoder_batch_complexity}
\end{equation}
The factor $B$ appears because, in the current implementation, each query in a batch separately constructs query-conditioned node inputs and performs graph encoding.
If query-independent structural gates for a fixed graph are cached during inference, part of the gate cost can be reduced; however, based on the current code implementation,
Eq.~\eqref{eq:encoder_batch_complexity} is a more conservative upper bound.

In the most common simplified analysis, we set $B=1$, $M=0$, disable dual branches, and regard the gating MLP as a lightweight constant-width module. Then
Eq.~\eqref{eq:encoder_batch_complexity} degenerates to
\begin{equation}
    O\left(L(md+d^2n)\right),
\end{equation}
which is exactly the core propagation complexity given in the main text. Here, $md$ corresponds to edge-level messages, structural gating, and sparse aggregation, while $d^2n$ corresponds to
node linear projection.

\subsection{Entity Scoring, Selector Regularization, and Document Projection Complexity}
\label{app:complexity_scoring_projection}

After GFM encoding obtains node representations, entity scoring is usually obtained by
\begin{equation}
    a_e(q)=\hh_e^\top \zz_q
\end{equation}
For one batch, the complexity of this step is
\begin{equation}
    C_{\mathrm{score}}(B)=O(Bnd).
\end{equation}
If the query-conditioned subgraph selector in Appendix~\ref{app:selector_regularizer} is enabled, then the additional inference-stage cost is
\begin{equation}
    C_{\mathrm{sel,infer}}(B)
    =
    O(Bnd^2+Bnd),
\end{equation}
which can be approximated as $O(Bnd)$ if the node-side projection is cached or a lightweight projection is used. During training, NCE, the size term, and the connectivity term also need to be computed,
with additional complexity
\begin{equation}
    C_{\mathrm{sel,train}}(B)
    =
    O(Bnd^2+Bnd+B^2d+Bm).
\end{equation}
Here, $B^2d$ comes from the in-batch query--subgraph contrastive matrix, and $Bm$ comes from the edge-level connectivity smoothing term.

Entity-to-document projection is performed by the entity--document matrix $\mathbf{M}$. If full sparse matrix multiplication is used, the complexity is
\begin{equation}
    C_{\mathrm{doc,full}}(B)
    =
    O\left(B\operatorname{nnz}(\mathbf{M})\right).
\end{equation}
The \texttt{IDFWeightedRanker} in the current code belongs to this type: it first constructs IDF weights according to entity occurrence frequency, and then performs
sparse matrix multiplication. If top-$K_e$ entity projection is used, conceptually only the inverted lists corresponding to these entities need to be accessed, so the complexity can be written as
\begin{equation}
    C_{\mathrm{doc,top}K}(B)
    =
    O\left(Bn\log K_e + B K_e\bar f\right),
    \label{eq:topk_doc_projection}
\end{equation}
where $Bn\log K_e$ comes from top-$K_e$ entity selection, and $BK_e\bar f$ comes from accessing the documents linked on average by the top entities.
If the final document top-$K$ ranking is performed over all $N_D$ documents, the complexity is $O(BN_D\log K)$; if it is performed only over the candidate document pool,
it is $O(BN_{\mathrm{cand}}\log K)$, where $N_{\mathrm{cand}}\ll N_D$.

\subsection{Training Complexity}
\label{app:complexity_training}

The main costs in the training stage come from GFM forward propagation, the entity-level retrieval loss, the optional selector regularizer, and backpropagation. Let
$\kappa_{\mathrm{bw}}$ denote the constant-factor cost of backpropagation relative to forward propagation, which can usually be regarded as a constant between $2$ and $3$.
If the entity-level training loss is BCE, ranking loss, or ListCE, then because the predicted scores of $n$ entities need to be supervised or ranked,
the loss computation complexity is
\begin{equation}
    C_{\mathrm{loss}}(B)=O(Bn).
\end{equation}
Therefore, when the selector is not enabled, the complexity of a single training batch is
\begin{equation}
    C_{\mathrm{train}}
    =
    O\left(
    \kappa_{\mathrm{bw}}
    \left[
        C_{\mathrm{enc}}(B)
        +
        C_{\mathrm{score}}(B)
        +
        C_{\mathrm{loss}}(B)
    \right]
    \right).
    \label{eq:train_complexity_no_selector}
\end{equation}
After enabling the query-conditioned subgraph selector, the training complexity becomes
\begin{equation}
    C_{\mathrm{train}}^{\mathrm{sel}}
    =
    O\left(
    \kappa_{\mathrm{bw}}
    \left[
        C_{\mathrm{enc}}(B)
        +
        C_{\mathrm{score}}(B)
        +
        C_{\mathrm{loss}}(B)
        +
        C_{\mathrm{sel,train}}(B)
    \right]
    \right).
    \label{eq:train_complexity_selector}
\end{equation}
If a document-level loss is also explicitly added during training, then entity-to-document projection needs to be additionally performed, with cost
$C_{\mathrm{doc,full}}(B)$ or $C_{\mathrm{doc,top}K}(B)$.

\subsection{Inference Complexity}
\label{app:complexity_inference}

The inference stage first performs query encoding, named entity recognition, and entity linking, whose total cost is denoted as
$C_{\mathrm{prep}}(q)$. This part depends on the adopted text encoder, NER model, and entity linking model, and does not belong to the graph propagation backbone.
Given the prepared query embedding and query entity mask, the core reading complexity of a single query is
\begin{equation}
\begin{aligned}
    C_{\mathrm{infer}}(q)
    =
    &(M+1)
    \Big[
        C_{\mathrm{enc}}(1)
        +
        C_{\mathrm{score}}(1)
        +
        C_{\mathrm{sel,infer}}(1)
        +
        C_{\mathrm{doc}}(1)
    \Big] \\
    &+
    C_{\mathrm{fuse}}(M,K),
\end{aligned}
\label{eq:inference_complexity}
\end{equation}
where $M$ is the number of pseudo-queries, $C_{\mathrm{doc}}(1)$ can take the complexity of full sparse projection or top-$K_e$ inverted projection,
and $C_{\mathrm{fuse}}(M,K)$ is the cost of fusing the results from the main query and pseudo-queries. If each query keeps $K$ candidate documents, then the cost of simple weighted
merging is
\begin{equation}
    C_{\mathrm{fuse}}(M,K)
    =
    O((M+1)K\log((M+1)K)),
\end{equation}

\subsection{Space Complexity}
\label{app:complexity_memory}

The model parameter space mainly comes from the GFM backbone, structural prompts, the structurally gated MLP, selector projections, and text projection layers. If we only discuss graph-
related runtime space, offline graph storage requires
\begin{equation}
    O\left(n+m+\operatorname{nnz}(\mathbf{M})+np_n+mp_e+p_g\right).
\end{equation}
During training, node activations of each layer need to be saved, and the space complexity is on the order of
\begin{equation}
    O(BLnd)
\end{equation}
If structurally gated edge messages are fully materialized, they require $O(md)$ GPU memory; the current implementation adopts edge chunk streaming.
Let the chunk size be $c$, then the peak memory of gated messages can be reduced to
\begin{equation}
    O(cd),
\end{equation}
where $c\ll m$. This is also one of the key engineering designs that makes the current implementation suitable for large-graph reading. If \texttt{return\_gate} is enabled and
the gate vectors of all edges are saved for visualization or interpretation, then the space will rise again to $O(md)$. If document scoring materializes all
$N_D$ document scores, it requires $O(BN_D)$ space; if only a candidate document heap is maintained, it can be reduced to $O(BK)$ or
$O(BK_e\bar f)$.

\subsection{Complexity Comparison with Related Work}
\label{app:complexity_related_work}

\paragraph{Overall Comparison.}
From the perspective of complexity, standard dense RAG has the lightest online retrieval cost, but it is difficult to explicitly model cross-document relations; multi-step RAG improves complex reasoning ability through multiple rounds of
retrieval, but its cost grows linearly with the number of LLM calls; GraphRAG-style methods shift a large amount of cost to offline graph construction
and summary generation; SubgraphRAG reduces online cost through lightweight triple scoring, but its effectiveness depends on the candidate triple set and structural distance features;
GFM-RAG and our reader concentrate the main computation on one or a small number of query-conditioned graph propagations.
Therefore, when the self-evolving memory loop needs to repeatedly evaluate the retrievability of different written graphs, the advantage of our design lies in the following:
each evaluation does not need to start multi-round LLM agentic search, but instead quickly obtains differentiable or scoreable retrieval feedback through a fixed GFM reader, structurally gated propagation, and sparse document projection.
This allows the graph writing strategy to perform high-frequency comparison and optimization over a large number of candidate memory graphs.

==> knowledge-intensive.tex <==
\begin{table*}[!t]
\centering
\footnotesize
    \caption{
    Overall results of~\model and baselines on five knowledge-intensive benchmarks in training-free and trainable RAG settings. We re-implement baselines and report their performance as the higher one between the original scores and our reproduced results. {*} indicates the results copied from~\cite{asai2023self} for reference. ``--'' indicates the  results are not reported in the original paper or not applicable (\eg, some methods cannot produce citations). The best performance is highlighted in {\bf \emph{bold}.}\label{tab:main}} 
    \vspace{-.5em}
\begin{tabular}{lccccccc}
\toprule
& PopQA & TriviaQA & NQ & MultiHopQA & \multicolumn{3}{c}{ASQA} \\ 
Method & (acc) & (acc) & (acc) & (acc) & (em) & (pre) & (rec)  \\ 
\midrule
\multicolumn{8}{c}{\it Baselines w/o Retrieval} \\
\multicolumn{8}{l}{\bf Vanilla Zero-shot Prompting} \\
\quad ChatGPT{*}  & {\color{gray}29.3} & {\color{gray}74.3} & -- & -- &  {\color{gray}35.3} & -- & --  \\
\quad Llama-3-Instruct$_{\textsc{8b}}$  
& 22.8 & 69.4 & 46.6 & 45.6 & 30.6 & -- & -- \\
\quad Llama-3-Instruct$_{\textsc{70b}}$  
& 28.9 & 80.6 & 57.9 & 57.5 & 39.1 & -- & -- \\
\midrule

\multicolumn{8}{c}{\it RAG w/o Training} \\
% {\bf In-Context RALM}~\citep{ram2023context} \\
\multicolumn{8}{l}{{\bf In-Context RALM}~\citep{ram2023context}} \\

\quad ChatGPT{*}  
& {\color{gray}50.8} & {\color{gray}65.7} & -- & -- &  {\color{gray}40.7} & {\color{gray}65.1} & {\color{gray}76.6}  \\
\quad Llama-3-Instruct$_{\textsc{8b}}$  
& 62.3 & 71.4 & 56.8 & 43.4 & 40.0 & 62.1 & 66.4 \\
\quad Llama-3-Instruct$_{\textsc{70b}}$  
& 63.8 & 76.3 & 60.2 & 51.2 & 43.1 & 62.9 & 67.6 \\
{\bf Few-Shot Demo. w/ Instruction} \\
\quad Llama-3-Instruct$_{\textsc{8b}}$
& 63.1 & 74.2 & 60.1 & 45.3 & 42.6 & 55.0 & 64.4 \\
\quad Llama-3-Instruct$_{\textsc{70b}}$ 
& 63.9 & 79.1 & 62.9 & 53.9 & 45.4 & 49.3 & 57.1 \\
{\bf \model-ICL} \\
\quad Llama-3-Instruct$_{\textsc{8b}}$
& 64.2 & 76.8 & 62.1 & 50.4 & 44.7 & {\bf 70.9} & {\bf 74.1} \\
\quad Llama-3-Instruct$_{\textsc{70b}}$
& {\bf 65.5} & {\bf 81.2} & {\bf 66.5} & {\bf 57.3}  & {\bf 47.8}  & 69.1 & 71.2 \\
\midrule

\multicolumn{8}{c}{\it RAG w/ Training} \\
{\bf Vanilla Supervised Fine-tuning} \\
\quad Llama-3-Instruct$_{\textsc{8b}}$  
& 61.0 & 73.9 & 56.6 & 56.1   & 43.8 & -- & --    \\
{\bf Self-RAG}~\citep{asai2023self} \\
\quad Llama-2$_{\textsc{7b}}$
& 55.8 & 68.9 & 42.4 & 35.9  & 30.0 & 66.9 & 67.8\\
\quad Llama-2$_{\textsc{13b}}$
& 56.3 & 70.4 & 46.4 & 36.0  & 31.4 & {\bf 70.3} & {\bf 71.3} \\
\quad Llama-3-Instruct$_{\textsc{8b}}$
& 55.8 & 71.4  & 42.8 & 32.9 & 36.9 & 69.7 & 69.7  \\
{\bf RetRobust}~\citep{yoranmaking2024} \\
\quad Llama-2$_{\textsc{13b}}$
& -- & -- & 39.6 & 51.5  & -- & -- & -- \\
\quad Llama-3-Instruct$_{\textsc{8b}}$
& 56.5 & 71.5 & 54.2 & 54.7  & 40.5 & -- & -- \\
{\bf \model-FT} \\
\quad Llama-3-Instruct$_{\textsc{8b}}$
& {\bf 66.2} & {\bf 78.5} & {\bf 65.7} & {\bf 57.2}  & {\bf 47.6} & 65.7 & 70.5 \\
%Relative Improvement & {\bf 66.2} ($\uparrow 8.5\%$) & {\bf 78.5} ($\uparrow 6.2\%$) & {\bf 65.7} ($\uparrow 16\%$) & {\bf 57.2} ($\uparrow 2\%$)  & {\bf 47.6} ($\uparrow 8.7\%$) & 65.7 & 70.5 \\
\bottomrule
\end{tabular}
\vspace{-1.5em}
\end{table*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

